Learn Locally, Correct Globally: A Distributed Algorithm for Training Graph Neural Networks

Despite the recent success of Graph Neural Networks (GNNs), training GNNs on large graphs remains challenging. The limited resource capacities of the existing servers, the dependency between nodes in a graph, and the privacy concern due to the centralized storage and model learning have spurred the need to design an effective distributed algorithm for GNN training. However, existing distributed GNN training methods impose either excessive communication costs or large memory overheads that hinders their scalability. To overcome these issues, we propose a communication-efficient distributed GNN training technique named $\text{{Learn Locally, Correct Globally}}$ (LLCG). To reduce the communication and memory overhead, each local machine in LLCG first trains a GNN on its local data by ignoring the dependency between nodes among different machines, then sends the locally trained model to the server for periodic model averaging. However, ignoring node dependency could result in significant performance degradation. To solve the performance degradation, we propose to apply $\text{{Global Server Corrections}}$ on the server to refine the locally learned models. We rigorously analyze the convergence of distributed methods with periodic model averaging for training GNNs and show that naively applying periodic model averaging but ignoring the dependency between nodes will suffer from an irreducible residual error. However, this residual error can be eliminated by utilizing the proposed global corrections to entail fast convergence rate. Extensive experiments on real-world datasets show that LLCG can significantly improve the efficiency without hurting the performance.

==> appendices/01.notation.tex <==
\section{Summary of notation}

We summarized all notations used throughout the paper in Table~\ref{table:notations}.

\input{tables/notations}

==> appendices/04.gradient_difference.tex <==
\clearpage
\section{Proof of Lemma~\ref{lemma:local_machine_structure_err}}


Let consider a single layer GNN with the loss $\mathcal{L}(\bm{\theta})$ and the gradient $\nabla \mathcal{L}(\bm{\theta})$ computed by 
\begin{equation}
    \begin{aligned}
    \mathcal{L}(\bm{\theta}) &= \frac{1}{N}\sum_{i\in\mathcal{V}} \ell(\mathbf{h}_i, y_i),~
    \mathbf{h}_i = \mathbf{W}^\top \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j,~\\
    \nabla \mathcal{L}(\bm{\theta}) &= \frac{1}{N}\sum_{i\in\mathcal{V}} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big).
    \end{aligned}
\end{equation}

When each local machine has access to the full graph structure and all other node features and suppose each local machine has the same number of nodes, we have 
\begin{equation}
    \nabla \mathcal{L}(\bm{\theta}) = \frac{1}{P}\sum_{p=1}^P \nabla \mathcal{L}_p^\text{full}(\bm{\theta}),~
    \nabla \mathcal{L}_p^\text{full} (\bm{\theta}) = \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big).
\end{equation}

However, in practice each local machine only have access to the node feature and graph structure on its local machine, i.e.,
\begin{equation}
    \nabla \mathcal{L}_p^\text{local} (\bm{\theta}) = \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\tilde{\mathbf{h}}_i, y_i)}{\partial \tilde{\mathbf{h}}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big).
\end{equation}


Define the local neighbor of node $v_i$ on machine $p$ by 
\begin{equation}
    \mathcal{N}^p(v_i) = \{ v_j|(v_i, v_j) \in \mathcal{E}_p\}.
\end{equation}


Let consider the neighbor average aggregation, where $L_{i,j}^p = \frac{1}{|\mathcal{N}^p(v_i)|}$ and $L_{i,j} = \frac{1}{|\mathcal{N}(v_i)|}$, we can upper bound $\mathbb{E}[ \| \tilde{\mathbf{h}}_i - \mathbf{h}_i \| ]$ by
\begin{equation}\label{eq:one_layer_example_eq_1}
    \mathbb{E}[ \| \tilde{\mathbf{h}}_i - \mathbf{h}_i \| ] \leq \mathbb{E} \Big[ \Big\| \mathbf{W}^\top \sum_{j \in \mathcal{V}_p} L_{i,j}^\text{local} \mathbf{x}_j - \mathbf{W}^\top \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big\| \Big] \leq D_\sigma B_w.
\end{equation}


To upper bound $\mathbb{E}[\| \nabla \mathcal{L}_p^\text{local}(\bm{\theta}) - \nabla \mathcal{L}_p^\text{full}(\bm{\theta}) \|^2]$, we have
\begingroup
\allowdisplaybreaks
    \begin{align*}
    & \mathbb{E}[\| \nabla \mathcal{L}_p^\text{local}(\bm{\theta}) - \nabla \mathcal{L}_p^\text{full}(\bm{\theta}) \|^2] \\
    &= \mathbb{E}\Big[\Big\| \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\tilde{\mathbf{h}}_i, y_i)}{\partial \tilde{\mathbf{h}}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) - \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    %======
    &\leq 2 \mathbb{E} \Big[ \Big\| \frac{P}{N} \sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\tilde{\mathbf{h}}_i, y_i)}{\partial \tilde{\mathbf{h}}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) - \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    &\quad + 2\mathbb{E} \Big[ \Big\| \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) - \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    %=======
    &\leq 2\mathbb{E} \Big[ \Big\| \frac{P}{N} \sum_{i\in\mathcal{V}_p} \Big( \frac{\partial\ell(\tilde{\mathbf{h}}_i, y_i)}{\partial \tilde{\mathbf{h}}_i} - \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big) \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    &\quad + 2\mathbb{E} \Big[ \Big\| \frac{P}{N}\sum_{i\in\mathcal{V}_p} \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j - \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    %=======
    &\leq \frac{2P}{N} \sum_{i \in \mathcal{V}_p} \mathbb{E} \Big[ \Big\| \Big( \frac{\partial\ell(\tilde{\mathbf{h}}_i, y_i)}{\partial \tilde{\mathbf{h}}_i} - \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big) \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    &\quad + \frac{2P}{N} \sum_{i \in \mathcal{V}_p} \mathbb{E} \Big[ \Big\| \frac{\partial\ell(\mathbf{h}_i, y_i)}{\partial \mathbf{h}_i} \Big( \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j - \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big) \Big\|^2 \Big] \\
    %=======
    &\underset{(a)}{\leq} \frac{2P}{N} \sum_{i \in \mathcal{V}_p} L_\ell^2 \mathbb{E}[ \| \tilde{\mathbf{h}}_i - \mathbf{h}_i \|^2] \mathbb{E} \Big[ \Big\| \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j \Big\|^2 \Big] \\
    &\quad + \frac{2P}{N} \sum_{i \in \mathcal{V}_p} \rho_\ell^2 \mathbb{E} \Big[ \Big\| \sum_{j \in \mathcal{V}_p} L_{i,j}^p \mathbf{x}_j - \sum_{j \in \mathcal{V}} L_{i,j} \mathbf{x}_j \Big\|^2 \Big],
\end{align*}
where $(a)$ is due to Lipschitz and smoothness assumption of loss function.

Recall $L_{i,j}^\text{local} = \frac{1}{|\mathcal{N}^\text{local}(v_i)|}$ and $L_{i,j} = \frac{1}{|\mathcal{N}(v_i)|}$, by plugging in Eq.~\ref{eq:one_layer_example_eq_1}, we can upper bound $\mathbb{E}[\| \nabla \mathcal{L}_p^\text{local}(\bm{\theta}) - \nabla \mathcal{L}_p^\text{full}(\bm{\theta}) \|^2]$ by
\begin{equation}
    \mathbb{E}[\| \nabla \mathcal{L}_p^\text{local}(\bm{\theta}) - \nabla \mathcal{L}_p^\text{full}(\bm{\theta}) \|^2] \leq 2 L_\ell^2 B_w^2 B_x^2 D_\sigma^2 + 2 \rho_\ell^2 D_\sigma^2.
\end{equation}



==> tables/datasets.tex <==
\begin{table}[h]
\centering
\vspace{-10pt}
\caption{Summary of datasets statistics. $\ddag$ indicates multi-labels dataset.}
\label{table:datasets}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}lllcccc@{}} \toprule
\textbf{Dataset}                            & \textbf{Nodes} & \textbf{Edges}   & \textbf{Feature}  & \textbf{Classes}  & \textbf{Train / Validation / Test} \\ \midrule % & \textbf{SOTA F1}\\ \midrule
\texttt{Flickr}~\cite{zeng2019graphsaint}   & $89,250$       & $899,756$        & $500$             & $7$               & 50\%~/~25\%~/~25\%                 \\ % & $51.6$~\cite{zeng2019graphsaint} \\ 
\texttt{OGB-Proteins}~\cite{hu2020open}     & $132,534$      & $39,561,252$     & $8$               & $112^{\bm\ddag}$  & 65\%~/~16\%~/~19\%                 \\ % & $79.2$~\cite{lb}                 \\ 
\texttt{OGB-Arxiv}~\cite{hu2020open}        & $169,343$      & $1,166,243$      & $12$              & $40$              & 54\%~/~17\%~/~28\%                 \\ % & $72.7$~\cite{lb}                 \\
\texttt{Reddit}~\cite{hamilton2017inductive}& $232,965$      & $11,606,919$     & $602$             & $41$              & 66\%~/~10\%~/~24\%                 \\ % & $96.6$~\cite{zeng2019graphsaint} \\ 
\texttt{Yelp}                               & $716,847$      & $13,954,819$     & $300$             & $100^{\bm\ddag}$  & 75\%~/~15\%~/~10\%                 \\ % & $63.8$~\cite{zeng2019graphsaint} \\
% \texttt{OGB Products}   & $2,449,029$    & $61,859,140$     & $100$             & $47$              & \phantom{0}8\%~/~\phantom{1}2\%~/~90\% & SAGE       \\ %& $75.6$~\cite{lb}
\bottomrule
\end{tabular}
}
\end{table}

%\texttt{OGB Mag}        & 1,939,743      & 21,111,007       & ?                 & ?                 & ?                                  & $4?.?$~\cite{lb}                 \\
%\texttt{OGB Papers100M} & $111,059,956$  & 1,615,685,872$  & $?$               & ?                 & ?                                  & GCN            & $66.4$                           \\
% \texttt{Amazon}         & 1,598,960      & 264,339,468      & 200               & $107$             & 78\%~/~\phantom{0}5\%~/~15\%       & $81.5$~\cite{zeng2019graphsaint} \\ 
% \texttt{OGB MAG240MLSC} & 244,160,499    & 1,728,364,232    & ?                 & ?                 & ?                                  &                                  \\ 

==> tables/notations.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{table*}[h]
\caption{Summary of notations used in this paper}
\label{table:notations}
\centering
\begin{tabularx}{\textwidth}{@{}sX@{}} \toprule
    $\mathcal{G}=(\mathcal{V},\mathcal{E})$  & $\mathcal{G}$ denotes the graph consist of set of $N=|\mathcal{V}|$ nodes and $M=|\mathcal{E}|$ edges. \\ \hline
    $\mathbf{A}, \mathbf{A}_p$ & $\mathbf{A}$ denotes the adjacency matrix corresponding to the graph $\mathcal{G}$, similarly $\mathbf{A}_p$ is the adjacency of subgraph on worker $p$ \\ \hline
    $\mathbf{D}$ & Denotes the degree matrix corresponding to the graph $\mathcal{G}$. \\ \hline
    $\mathbf{L}$, $\mathbf{L}^{p}$ & $\mathbf{L}$ denotes the full Laplacian matrix calculated by $\mathbf{L}=\mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$ and $\mathbf{L}^{p}$ is the Laplacian matrix for the local subgraph on worker $p$. \\ \hline
    $\mathbf{X}$, $\bm{x}_i$ & $\mathbf{X}$ denotes the node feature matrix for all $N$ nodes where $\mathbf{X}=[\bm{x}_1,\ldots,\bm{x}_N]$. \\ \hline
    $\mathbf{Y}, \bm{y}_i$ & $\mathbf{Y}$ denotes the stacked label features and $\bm{y}_i$ denotes the label vector in $\mathbb{R}^C$. For example, in binary classification task, $\bm{y}_i\in\mathbb{R}^C$ is a one-hot vector with $C=2$.   \\ \hline
    $\mathbf{H}^{(\ell)},\mathbf{Z}^{(\ell)}$ & $\mathbf{Z}^{(\ell)}$ denotes the node feature matrix for the $\ell$th layer before activation and $\mathbf{H}^{(\ell)} = \sigma(\mathbf{Z}^{(\ell)})$ denotes the node feature matrix after the $\ell$th layer. \\ \hline
    $\mathbf{W}^{(\ell)}, \bm{\theta}$ $\mathbf{W}_p^{(\ell)}, \bm{\theta}_p$ & {$\mathbf{W}^{(\ell)}$ denotes the weight matrix for the $\ell$th graph convolution layer, $\bm{\theta}:=\{\mathbf{W}^{(1)},\ldots,\mathbf{W}^{(L)}\}$ denotes the stacked parameters. Per worker weight matrix and parameters are defined respectively.} \\ \hline
    $\kappa$ & The residual error as a result of applying naive parameter averaging in distributed GCNs. \\ \hline
    $P, T, K, S $ & $P$ denotes the number of local workers and $T$ is the total number of SGD updates. $K$ denotes the number of local worker iterations and $S$ is number of server correction iterations per epoch.\\ \hline
    $\mathcal{L}(\bm{\theta}), \mathcal{L}_p^\text{local}(\bm{\theta})$ $\mathcal{L}_p^\text{full}(\bm{\theta})$ &  $\mathcal{L}(\bm{\theta})$ denotes the objective on the global graph, $\mathcal{L}_p^\text{local}(\bm{\theta})$ denotes the local objective on the local subgraph and $\mathcal{L}_p^\text{full}(\bm{\theta})$ is the local objective with access to the global graph. \\ \hline
    $\mathcal{N}{(v_i)}, \mathcal{N}_p{(v_i)}$ & Denote the neighbor of node $v_i$ on the global graph and local graph respectively \\ \hline
    $\eta, \gamma$ & Learning rate on the server and local workers, respectively.  \\ \hline 
    $\sigma(\cdot)$ & $\sigma(\cdot)$ is the activation function, e.g., ReLU function. \\\hline
    $\phi(\cdot, \bm{y}_i)$ & $\phi(\cdot,\bm{y}_i)$ is the loss function, e.g., cross-entropy loss
    \begin{equation*}
    \phi(\bm{z}_i, \bm{y}_i) = -\log\left(\frac{\exp( \bm{z}_i^\top {\bm{y}_i})}{\sum_{j=1}^C \exp([\bm{z}_i]_j))}\right),
    \end{equation*}
    where label vector $\bm{y}_i$ is a one-hot vector. \\
    \bottomrule
\end{tabularx}
\end{table*}

==> tables/w_llgc.tex <==
\begin{algorithm}[h]
 \caption{Distributed Training of GCN with \textbf{Correction}}
 \label{alg:distgnn-corr-2}
%  \begin{algorithmic}[1]
%     \Require 
%     % Number of layers $L$,
%     Input graph $\mathbf{A}\in\mathbb{R}^{N\times N}$, 
%     node features $\mathbf{X}\in\mathbb{R}^{N\times d}$,
%     labels $\mathbf{Y}\in\mathbb{R}^{N\times C}$,
%     their partitioned counterparts $\mathbf{A}_p$, $\mathbf{X}_p$, $\mathbf{Y}_p$, 
%     global initial parameters $\bar{\boldsymbol{\theta}}^0$ and
%     local parameters $\boldsymbol{\theta}^0_p$.
%     \textcolor{red}{$K$ local update size, $\rho$ growth rate, $S$ global steps}
%     \For {$r$}{$1$}{$R$}
%         % \ForP {$p$}{$1$}{$P$} \Comment{In Parallel}
%             \State Each worker $p$ sends the local parameters $\boldsymbol{\theta}^t_p$ to the server
%             \State Server updates the global parameters by parameter average $\bar{\boldsymbol{\theta}}^t = \frac{1}{P}\sum_{p=1}^{P} \boldsymbol{\theta}^t_p$
%             \State Each worker $p$ receives the global parameters from server $\boldsymbol{\theta}^t_p \gets \bar{\boldsymbol{\theta}}^t$
%             %
%             % \If{$t~\text{mod}~(K+S) \in \{ 1, \ldots, K \}$}
%             \For{$k$}{$1$}{$K \rho^r$}
%                 \State $t=k + \frac{K(1-\rho^{r-1})}{1-\rho} + S(r-1)$
%                 \ForP {$p$}{$1$}{$P$}
%                     \State Train GNN using $\mathbf{A}_p$ and $\mathbf{X}_p$ \Comment{Forward pass}
%                     \State Compute loss and the gradients using $\mathbf{Y}_p$ \Comment{Backward pass}
%                     \State Update the local parameters $\boldsymbol{\theta}^t_p$ with learning rate $\eta$
%                 \EndFor
%             \EndFor
%             % \ElsIf{$t~\text{mod}~(K+S) \in \{K+1, \ldots, K+S\}$}
%             \For{$s$}{$1$}{$S$}
%                 \State $t=s + \frac{K(1-\rho^{r})}{1-\rho} + S(r-1)$
%                 \State Sample a snapshot of $\mathbf{A}$, $\mathbf{X}$, $\mathbf{Y}$
%                 \State Update the global parameters $\bar{\boldsymbol{\theta}}^t$ with learning rate $\gamma$
%             % \EndIf
%             \EndFor
%     \EndFor
%     \Ensure \texttt{GCN} model with trained $\bar{\boldsymbol{\theta}}^{T+1}$
% \end{algorithmic}
\begin{algorithmic}[1]
    \Require 
    % Number of layers $L$,
    Input graph adjacency $\mathbf{A}\in\mathbb{R}^{N\times N}$, 
    node features $\mathbf{X}\in\mathbb{R}^{N\times d}$,
    labels $\mathbf{Y}\in\mathbb{R}^{N\times C}$,
    their partitioned counterparts $\mathbf{A}_p$, $\mathbf{X}_p$, $\mathbf{Y}_p$, 
    global initial parameters $\bar{\boldsymbol{\theta}}^0$ and
    local parameters $\boldsymbol{\theta}^0_p$
    \State $t \gets 0$
    \For {$r$}{$1$}{$R$}
        % \ForP {$p$}{$1$}{$P$} \Comment{In Parallel}
        \tikzmk{A}
        \ForP {$p$}{$1$}{$P$} \Comment{Local Learning}
            \State Worker $p$ receives the global parameters $\boldsymbol{\theta}^{t}_p \gets \bar{\boldsymbol{\theta}}^t$ \Comment{Communication}
            \For {$k$}{$1$}{$\rho^rK$}
                \State $t \gets t + 1$
                \State Construct the mini-batch $\xi_p^t$ using $\mathbf{A}_p$ and $\mathbf{X}_p$
                \State Compute hidden embedding $\mathbf{H}^{(\ell)}_p$ and stochastic gradients $\tilde{\nabla} \mathcal{L}_p^\text{local}(\bm{\theta}_p^t, \xi_p^t)$ % using Eq.~\ref{eq:update_rule_convergence}
                \State Update model parameter by $\boldsymbol{\theta}^{t}_p =  \boldsymbol{\theta}^{t-1}_p - \eta \tilde{\nabla} \mathcal{L}_p^\text{local}(\bm{\theta}_p^t, \xi_p^t)$
            \EndFor
            \State Worker $p$ sends the local parameters $\boldsymbol{\theta}^t_p$ to the server \Comment{Communication}
        \EndFor \tikzmk{B}\boxitf{codell}
        \State Server updates the global parameters using parameter averaging $\bar{\boldsymbol{\theta}}^t = \frac{1}{P}\sum_{p=1}^{P} \boldsymbol{\theta}^t_p$
        \tikzmk{A}
        \For {$s$}{$1$}{$S$} \Comment{Server Correction}
            \State $t \gets t + 1$
            \State Construct the snapshot $\xi^t$ using $\mathbf{A}$ and $\mathbf{X}$ %, $\mathbf{Y}$
            \State Compute hidden embedding using and the stochastic gradient $\tilde{\nabla} \mathcal{L}(\bar{\bm{\theta}}^t, \xi^t)$ % Eq.~\ref{eq:update_rule_convergence_server}
            \State $\bar{\boldsymbol{\theta}}^{t} =  \bar{\boldsymbol{\theta}}^{t-1} - \gamma \tilde{\nabla} \mathcal{L}(\bar{\bm{\theta}}^t, \xi^t)$
        \EndFor \tikzmk{B} \boxits{codecg}
    \EndFor
    \Ensure \texttt{GCN} model with trained $\min_t \mathbb{E}[ \| \nabla \mathcal{L}(\bar{\boldsymbol{\theta}}^{t}) \|^2 ]$
\end{algorithmic}
\end{algorithm} 
